Scaling pair count to next galaxy surveys

Counting pairs of galaxies or stars according to their distance is at the core of real-space correlation analyzes performed in astrophysics and cosmology. Upcoming galaxy surveys (LSST, Euclid) will measure properties of billions of galaxies challenging our ability to perform such counting in a minute-scale time relevant for the usage of simulations. The problem is only limited by efficient access to the data, hence belongs to the big data category. We use the popular Apache Spark framework to address it and design an efficient high-throughput algorithm to deal with hundreds of millions to billions of input data. To optimize it, we revisit the question of nonhierarchical sphere pixelization based on cube symmetries and develop a new one dubbed the "Similar Radius Sphere Pixelization" (SARSPix) with very close to square pixels. It provides the most adapted indexing over the sphere for all distance-related computations. Using LSST-like fast simulations, we compute autocorrelation functions on tomographic bins containing between a hundred million to one billion data points. In each case we achieve the construction of a standard pair-distance histogram in about 2 minutes, using a simple algorithm that is shown to scale, over a moderate number of nodes (16 to 64). This illustrates the potential of this new techniques in the field of astronomy where data access is becoming the main bottleneck. They can be easily adapted to other use-cases as nearest-neighbors search, catalog cross-match or cluster finding. The software is publicly available from https://github.com/astrolabsoftware/SparkCorr.

==> abstract.tex <==
Counting pairs of galaxies or stars according to their
distance is at the core of real-space correlation analyzes performed in astrophysics and cosmology.
Upcoming galaxy surveys (LSST, Euclid) will measure properties of  billions of galaxies
challenging our ability to perform such counting in a minute-scale time relevant for the usage of simulations. 
The problem is only limited by efficient
access to the data, hence belongs to the big data category.
We use the popular Apache Spark framework to address it and design an
efficient high-throughput algorithm to deal with hundreds of millions to
billions of input data.
To optimize it, we revisit the question of nonhierarchical sphere pixelization
based on cube symmetries and develop a new one dubbed the "Similar
Radius Sphere Pixelization" (SARSPix) with very close to square pixels.
It provides the most adapted indexing over the sphere for all distance-related computations.
Using LSST-like fast simulations, we compute autocorrelation
functions on tomographic bins containing between a hundred million to
one billion data points. In each case we achieve the construction
of a standard pair-distance histogram in about 2 minutes, using a
simple algorithm that is shown to scale, over a moderate number of nodes (16 to 64). 
This illustrates the potential of
this new techniques in the field of astronomy where data access is
becoming the main bottleneck. They can be easily adapted to other use-cases as
nearest-neighbors search, catalog cross-match or cluster finding.
The software is publicly available from https://github.com/astrolabsoftware/SparkCorr.

